Video Rescaling Networks with Joint Optimization Strategies for Downscaling and Upscaling

This paper addresses the video rescaling task, which arises from the needs of adapting the video spatial resolution to suit individual viewing devices. We aim to jointly optimize video downscaling and upscaling as a combined task. Most recent studies focus on image-based solutions, which do not consider temporal information. We present two joint optimization approaches based on invertible neural networks with coupling layers. Our Long Short-Term Memory Video Rescaling Network (LSTM-VRN) leverages temporal information in the low-resolution video to form an explicit prediction of the missing high-frequency information for upscaling. Our Multi-input Multi-output Video Rescaling Network (MIMO-VRN) proposes a new strategy for downscaling and upscaling a group of video frames simultaneously. Not only do they outperform the image-based invertible model in terms of quantitative and qualitative results, but also show much improved upscaling quality than the video rescaling methods without joint optimization. To our best knowledge, this work is the first attempt at the joint optimization of video downscaling and upscaling.

==> tables/mean.tex <==
\begin{table}[t]\centering
\setlength{\tabcolsep}{4.5pt}
\caption{Ablation study on high-frequency information $z$}
\begin{tabular}{c|c|c}
\hline
Method & Predicted  & HR PSNR\\ \hline
LSTM-VRN &  & 27.46\\
LSTM-VRN & $\surd$ & 32.18 \\
\hline
MIMO-VRN &  & 25.89\\
MIMO-VRN & $\surd$ & 33.79 \\
\hline
\end{tabular}
\label{table:z}
\end{table}

==> tables/z.tex <==
\begin{table}[t]\centering
\setlength{\tabcolsep}{4.5pt}
\caption{Ablation study on the case of $\hat{z}$ for MIMO-VRN}
\begin{tabular}{c|c}
\hline
Case of $\hat{z}$  & HR PSNR-Y\\ \hline
Case-agnostic & 33.50\\
Case-specific & 33.79 \\
\hline
\end{tabular}
\label{table:z}
\end{table}

\begin{comment}
\begin{table}[t]\centering
\setlength{\tabcolsep}{4.5pt}
\caption{Ablation Study on high-frequency information $z$}
\begin{tabular}{c|c|c}
\hline
Method & Predictive Module  & HR PSNR\\ \hline
LSTM-VRN &  & 27.46\\
LSTM-VRN & $\surd$ & 32.18 \\
\hline
MIMO-VRN &  & 25.89\\
MIMO-VRN & $\surd$ & 33.79 \\
\hline
\end{tabular}
\label{table:z}
\end{table}
\end{comment}




\begin{comment}
\begin{table}[t]\centering
\setlength{\tabcolsep}{4.5pt}
\caption{Ablation Study on high-frequency information $z$}
\begin{tabular}{c|c|c}
\hline
Method & Generation of $z$  & HR PSNR\\ \hline
GoF5 zero & zero & 29.88\\
GoF5 & Predictive Module & 33.79\\
\hline
\end{tabular}
\label{table:z}
\end{table}
\end{comment}

==> tables/zeros.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{7pt}
\caption{The comparison of different method }
\begin{tabular}{c|ccccc}
\hline
Method & Predictive Module & HR PSNR-Y/SSIM-Y & LR PSNR-Y/SSIM-Y & HR VMAF & LR VMAF\\ \hline
IRN_Ret & & 30.72/0.9087 & 45.06/0.9908 & 86.37 & 95.55\\
LSTM-VRN & $\surd$ & 32.24/0.9369 & 42.36/0.9940 & 88.04 & 96.79 \\ \hline
MIMO-VRN-C zero & & 33.04/0.9575 & 45.49/0.9970 & 89.00 & 98.21\\
MIMO-VRN-C & $\surd$ & 33.40/0.9609 & 45.54/0.9969 & 89.64 & 98.33 \\
\hline
\end{tabular}
\label{table:zero}
\end{table*}

==> tables/zeros_irn.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{4.5pt}
\caption{Ablation study on the case of $\hat{z}$ for IRN. The results are evaluated on Vid4.}
\begin{tabular}{c|cc}
\hline
Case of $\hat{z}$  & HR PSNR-Y & LR PSNR-Y\\ \hline
Case-agnostic & 33.04 & 45.49\\
Case-specific & 33.40 & 45.54\\
\hline
\end{tabular}
\label{table:zero}
\end{table}
